FPRAS Approximation of the Matrix Permanent in Practice

The matrix permanent belongs to the complexity class #P-Complete. It is generally believed to be computationally infeasible for large problem sizes, and significant research has been done on approximation algorithms for the matrix permanent. We present an implementation and detailed runtime analysis of one such Markov Chain Monte Carlo (MCMC) based Fully Polynomial Randomized Approximation Scheme (FPRAS) for the matrix permanent, which has previously only been described theoretically and with big-Oh runtime analysis. We demonstrate by analysis and experiment that the constant factors hidden by previous big-Oh analyses result in computational infeasibility.

==> ack.tex <==
% \thispagestyle{empty}
\acknowledge
	I would like to thank my advisor and thesis committee chair, Dr. Moshe Vardi, for his guidance, support, and patience. His passion for teaching, for mentoring, and for computer science have been a continual inspiration.
	
	I would like to thank Dr. Luay Nakhleh and Dr. Krishna Palem for serving on my thesis committee.
	
	I would like to thank the Department of Computer Science and the Office of Graduate and Postdoctoral Studies at Rice University for accommodating the abrupt interruption in my studies that occurred following the very premature birth of my son. 
	
	Finally, I would like to thank my wife, Kathryn, without whose support and dedication my graduate studies would not have been possible.
\endacknowledge
